Dynamic Deformation of Uniform Elastic Two-Layer Objects

This thesis presents a two-layer uniform facet elastic object for real-time simulation based on physics modeling method. It describes the elastic object procedural modeling algorithm with particle system from the simplest one-dimensional object, to more complex two-dimensional and three-dimensional objects. The double-layered elastic object consists of inner and outer elastic mass spring surfaces and compressible internal pressure. The density of the inner layer can be set different from the density of the outer layer; the motion of the inner layer can be opposite to the motion of the outer layer. These special features, which cannot be achieved by a single layered object, result in improved imitation of a soft body, such as tissue's liquidity non-uniform deformation. The construction of the double-layered elastic object is closer to the real tissue's physical structure. The inertial behavior of the elastic object is well illustrated in environments with gravity and collisions with walls, ceiling, and floor. The collision detection is defined by elastic collision penalty method and the motion of the object is guided by the Ordinary Differential Equation computation. Users can interact with the modeled objects, deform them, and observe the response to their action in real time.

==> code.tex <==
\chapter{Related Work}
\label{chapt:related work}
\index{related work}

Research about modeling deformable objects in computer graphics field has been going on for over 40 years and a wide variety techniques have been developed. In this chapter, I will review the existing geometric approaches for modeling elastic objects. These models are all based on physical laws. From the early elastic model, such as particle model, mass-spring  model, finite element model, to recent development such as implicit surface model, fluid based model, and pressure model, I briefly introduce their physically-based modeling methods and compare these approaches with their advantages and disadvantages.



\section{Existing Elastic Object Models}

\paragraph*{Particle Model} has been used by Reeves\cite{TR83} and to model the natural phenomena such as fire, water, liquid. Particles move under the force field and constraint without interacting with each other. 
\begin{figure*}[h]
\begin{center}
	{\label{fig:particle}
	 \includegraphics[width=2in]{images/particle.png}}
\caption{Particle System}
\end{center}
\end{figure*}

%In another particel model, presented by Wyvill et al \cite{gw86}, the energy implicit functions to model the inter-particle connection are used with a large number of particles. (arranged themselves into volumes or surfaces?)

\paragraph*{Deformable Surface} was introduced first time by Terzopoulos et al \cite{tpb87}, using finite difference for the integration of energy-based Lagrange equations based on Hooke's law. It was very successful in creating and animating surfaces. However, this method requires not only the discretization of the surfaces into spline patches, but also the specification of local connectivity for spring mass systems. These involve a significant amount of manual preprocessing before the surface model can be used.

\paragraph*{Linear Mass Spring System} has been widely used for modeling elastic objects. It is actually derived from the particle model; however, it simplifies the modeling of the inter-particle connection by using flexible springs. Three dimensional systems contain a finite set of masses connected by springs, which obey Hooke's Law. 

%the cloth spring. Later, spring-mass based models\cite{gl99}.

\begin{figure*}[h]
\begin{center}
	{\label{fig:massspring}
	 \includegraphics[width=2in]{images/massspring.png}}
\caption{Mass-spring Model}
\end{center}
\end{figure*}

A very interesting application about this method was introduced by Terzopoulos\cite{TPF89} to describe melting effects. Particles, which are connected by springs, have an associated temperature as one of their properties. The stiffness of the spring is dependent on the temperature of the linked two particles. Increased temperature decreases the spring stiffness. When the temperature reaches the melting point, the stiffness becomes zero.

The advantages of mass-spring model are easy to construct and demonstrate the simulation dynamically. 

The disadvantages are that such system restricts to only the compressible object simulation of approximation of the true physics, not for the incompressible objects, and the separation and fusion of a constant volume object.  Moreover, the spring stiffness is problematic. If the spring is too soft, for the closed shape model with only simple springs to model the surface will be very easy to collapse. If we try to avoid the collapse, we need to model the spring more stiff, and then we will have difficulty to compromise the elasticity because the object is nearly rigid. Another disadvantage is that the mass spring system has less stability and require the numerical integrator to take small time steps\cite{BW92}. 

\paragraph*{Angular Springs With Stiff Distance Constraints} is similar to linear mass spring system; however, the force is applied based on angles between springs rather than distance between particles. In this system, mass distances are held constant by stiff springs.

\paragraph*{Discreet Force Field} presents a vector field of forces using a three dimensional array. Each particle in the system contributes repulsive and / or attractive forces to nearby force `elements' in the array. Later all of the particles have the force of their discrete force 'element' applied to them.


\paragraph*{FEM Model} known as Finite Element Method\cite{gm97}, is the most accurate physical model compared to other models. It treats deformable object as a continuum, which means the solid bodies with mass and energy distributed all over the object. This continuum model is derived from equations of continuum mechanics. The whole model can be considered as the equilibrium of a general object applied with external forces. The deformation of the elastic object is a function of these forces and the material property. The object will stop deformation and reach the equilibrium state when the potential energy is minimized. The applied forces must be converted to the associated force vectors and the mass and stiffness are computed by numerically integrating over the object at each time step, so the re-evaluation of the object deformation is necessary and require heavy pre-processing time. 

%based techniques (Fedkiw, 2003): 

The advantage of FEM model is that it is more realistic than mass-spring system because the physics are more accurate. It gives great results about the deformable modeling. 

The disadvantage is that the system lacks of efficiency. Because the energy equation will be used, so the FEM is only efficient for the small deformation of the elastic object, such as apply to the plastic material requires less deformation or the object consists less control elements needed to be computed. If we need to simulate the human soft part and facial animation, the deformation rate is very high. Therefore, it has been limited to apply in real-time system because of the heavy computation. Moreover, the implementation is complicated and the computation is slow. Usually it is off line.

\paragraph*{Fluid Based Model}\cite{ND02} consists of two components: an elastic surface and a compressible fluid. The surface is represented as a mass spring system. The fluid is modeled using finite difference approximations to the Navier-Stokes equations of fluid flow.
\begin{figure*}[h]
\begin{center}
	{\label{fig:fluid}
	 \includegraphics[width=2in]{images/fluid.png}}
\caption{Fluid-Based Soft-Object Model}
\end{center}
\end{figure*}

This figure shows the fluid flowing down a sink is simulated using a particle system.

The draw back of this model is the heavy computation for both elastic surface and density inside fluid. It also provides a solution to the constant volume problem.

\paragraph*{Pressure Model} was introduced by M. Matyka in 2003\cite{mm041, mm042, mm042}. It simulates an elastic deformable object with a internal pressure based on the ideal gas law. The object volume is approximately calculated by bounding box, shaped as sphere, cube, or ellipsoid. Another method to determine the object volume is based on Gauss Theorem.

\begin{figure*}[h]
\begin{center}
	{\label{fig:pressure}
	 \includegraphics[width=1.5in]{images/pressure.png}}
\caption{Pressure Soft Body Model}
\end{center}
\end{figure*}

Even though this model gives very convincing effects about elastic property in real time simulation, the object behaves as if a balloon filled only with air, which follows the physical law defined for the model itself. For more interesting effects, such as human tissue, it can not imitate. It can not achieve the effect of semi liquid deformable object because the air pressure density is unit inside of the object, which is different from liquid with non-unit density. It is not accurate for describing the inertia of the semi liquid object.

%\paragraph*{SPAM} Smooth-Particle Applied Mechanics
%can model both fluids and solids using free-moving particles.
%\section{Existing Physical Engine}

%Professional game physics engine Havok

%Virtual reality simulation engine Vortex
\section{Summary of The Existed Models}
Previous work on deformable object animation uses physically-based methods with local and global deformations applied directly to the geometric models. Based on the survey of the existed elastic models, I conclude their usage as the two types:
\begin{itemize}
\item Interactive models are used when speed and low latency are most important and physical accuracy is secondary. Typical examples include mass-spring models and spline surfaces used as deformable models. These can satisfy the character animation with exaggerated unrealistic deformation.
\item Accurate models are chosen when physical accuracy is important in order to accomplish the surgical training purpose which requires the accurate tissue modeling. The continuum simulation model, for instance, the most accurate model, FEM, is not ideal for simulation requiring real time interaction and the object undergoing large deformation. 
\end{itemize}

%When two flexible objects collide, they exert reaction forces on each other resulting in the deformation of both objects. When one object self collides, it may deform and result n self-intersection. 

In short, elastic object simulation is a dilemma of demanding accuracy and interactivity. 



==> design.tex <==
\chapter{Physical Based Numerical Integration Methodology}
\label{chapt:physical based numerical integration methodology}
\index{Physical Based Numerical Integration Methodology}

In chapter 3, I have introduced the geometric modeling method about the one-dimensional, two-dimensional, and three-dimensional elastic objects; more importantly, I have discussed the related forces, such as external gravity force, and the internal forces like spring force and pressure force accumulated on the object.

Assume, after the elastic object simulation system creates an elastic object with its initial state as Fig.\ref{fig:dt0}, the system starts the simulation. The simulation system is updated a finite number of times. The object is at the state in Fig.\ref{fig:dt100} after the updates of 50 discrete time steps.

\begin{figure*}[h]
\begin{center}
\subfigure[Elastic Object at the Initial Step]
	{\label{fig:dt0}
	 \includegraphics[width=2in]{images/dt0.png}}
	 \hspace{.6in}
	 	\subfigure[Elastic Object at the Step 50]
	{\label{fig:dt100}
	 \includegraphics[width=2in]{images/dt100.png}}
\caption{Elastic Object at Different Time States}
\end{center}
\end{figure*}

In each update, the accumulated impart forces on the particle tell it how to change the velocity for next step and result in a re-computation of the force.   The dynamic force applied on this object throughout the time passes may be the collision force when the object reaches the boundary; or, the mouse dragging force when user interacts with the object. Overall, the shape deformation of this soft body is also computed in real time. So, it is important to study the physical based mathematical theory, differential equations, in order to help us understand how the velocity and displacement of the object are integrated dynamically from the knowledge of force applied to it. 

\section{Differential Equations}
Differential equations describe such relation between a function and its one or more derivatives. The order of the equation is the order of the highest derivative it contains. The elastic object simulation system is more associated with the initial value problems. So, we will concentrate on ODE (ordinary differential equation), which uses linear extrapolation of the state variable, such as position and velocity, during the derivate of the state at discrete time steps.  
$$\dot{y} = f(y,t)$$ %= \frac{\partial x}{\partial t}$$

where

$f$ = a function that can evaluate the given $y$ and $t$
 
$y$ = is a vector, which is the state of the system

$\dot{y}$ = is a vector, which is $y$'s time derivative. 

$t = t_{0} + \partial t$  and $\partial t$ is the stepsize of time

$y(t_0) = $the initial state at the start point $t_0$ 

$y(t)$ = the value we need to find over time thereafter.

To solve a differential equation is to find a function that can satisfy this relation. In our elastic simulation system, the derivative of position is velocity and the derivative of velocity is acceleration.
$$\dot{x} = f(v, t)$$
$$\dot{v} = f(a, t) = f(f, t)$$
where 

$x$ is position, 

$v$ is velocity, 

$a$ is acceleration,and

$f$ is force.
%The velocity $v$ is the Differential Equations function of position x and time t; he force f is the Differential Equations function of position x and time t.  

%Simple scalar and vector calculus\cite{TF96} (derivatives and integrals)

Let's take one particle on the object as an example and understand how the different integrators work.
\section{Explicit Euler Integrator}

The simplest ODE integration method is Explicit Euler Integration method or Forward Euler method, which only evaluates derivatives, or called slope at the beginning of the interval and add it to the variable. Then redeterminie the slope of the curve and taking the next step along the new tangent. From the figure below, we can see the method is asymmetric according to the beginning and the end of the interval. It is a low accuracy prototype ODE.

\begin{figure*}[h]
\begin{center}
	{\label{fig:euler}
	 \includegraphics[width=3in]{images/euler.png}}
\caption{Euler Integrator}
\end{center}
\end{figure*}
\subsection{Theory}
Consider a Taylor series expansion as in Eq(\ref{eqn:Taylor}):

\begin{equation}
\label{eqn:Taylor}
y({t_0}+{\partial t}) = y({t_0}) + {\partial t}\dot{y}({t_0})+ \frac{{{\partial t}^2}{\ddot{y}}({t_0})}{2!}+\ddots+\frac{{{\partial t}^n}\left(\frac{\partial^{n}y}{\partial{t}^n}\right)}{n!}
\end{equation} 
%\begin{equation}
%\label{eq:Taylor}
%x({t}+{\partial t}) = x({t}) + {\partial t}\dot{x}({t})+ \frac{{{\partial t}^2}{\ddot{x}}({t})}{2!}+\ddots+\frac{{{\partial t}^n}\left(\frac{\partial^{n}x}{\partial{t}^n}\right)}{n!}
%\end{equation

then,

Euler method retains only first two derivative term:
%\begin{equation}
$$y({t_0}+{\partial t}) = y({t_0}) + {\partial t}\dot{y}({t})$$
%\end{equation} 
$$k_0 = y({t_0})$$
$$k_1 = {{\partial t}}\dot{y}({t}) = {\partial t}f(y,t) $$
$$y({t}+{\partial t}) = k_0 + k_1$$
where

$k_0$ is the initial state

$k_1$ is the function to find the simplest estimation, the Euler slope of the interval.
%where
%\begin{equation}
% y(t) =  y(t_0) + (t-t_0)f(t_0, y_0) 
%\end{equation}

%then
%\begin{eqnarray*}       
%y_1 = y_0 + \partial t f(y_0, t_0)\\    
%y_2 = y_0 + \partial t f(y_1, t_0)\\
%.....\\
%y_{j+1} = y_0 + \partial t f(y_j, t_0)\\
%\end{eqnarray*}       




%\begin{center}
%$y({t}+{h}) = {h}\dot{y}({t})$

%$k0 = y({t})$

%$k1 = {h}\dot{y}({t}) = {h}f(y,t)$

%$y({t}+{h}) = k0 + k1$

%formula $y_{n+1} = y_n {h}f(y_n,t_n)$
%\end{center}



%\section{Implicit methods} 

%formula $y_{n+1} = y_n {h}f(y_n,t_n)$

%Implicit method is also called backward Euler method, which is based on the explicit methods, sometimes, the ODE can become non accurate and do not provide a very good result. So, implicit method can be applied to solve the stability problem. This method can use the large step size. However, it is more expensive in time and space computation and difficult

%For spring mass: 
%$v(t+\partial t) = (v(t)-\partial t*SpringConstant/Mass*x(t) + \partial t*gravity) / (1 + \partial t*dt*SpringConstant/SpringMassMass) $

%$x(t+\partial t) = x + \partial t*v(t+\partial t) $

%If I set the spring coefficient value very high because I want very stiff springs, the little Euler integrator cannot handle it.
\subsection{Newton's Laws}
After the force accumulation on the object, it is important to find the acceleration because the force is not the only criteria to move the object. We have to define the relationship between position, velocity, and acceleration. The position, velocity, and acceleration of the particles is governed by Newton's law.  
\begin{diamonds}
\item Position: is the distance the object is away from the reference point, or is the direction relative to that reference point. 
\item Velocity: is the rate of change of position over time.
\item Acceleration: is the rate of change of velocity.
\item Derivative of Position: is the velocity and defines the rate at velocity changes and tells us what direction and how fast it is moving.
\item Derivative of Velocity: is the acceleration and defines the rate at acceleration changes.
\end{diamonds}


%\begin{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Netwon's 2nd law F = ma
%\item

Given
a set of forces acting on a particle ${F}$ at time $t$,
the mass  of the particle ${m}$, and
the constant acceleration of the particle ${a}$, and as
the Newton's 2nd law, with real time force ${F}$ on the particle.
The directly affect to the force is the acceleration which can be represented with the relation of force and its mass:

\begin{equation}
{F} = {m}{a} \Rightarrow {a}=\frac{F}{m}
\label{equ:ising}
\end{equation}

Also, the acceleration can be defined as the rate of change with respect
to time of the velocity $v$ of the particle, assuming $v$ is constant. 
Under that assumption we can also compute the position $x$ of a particle.

\begin{equation}
{v} = {a}{t} ; {x} = {v}{t}
\end{equation}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%     get the acceleration a = F/m     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\item
%\begin{equation}
%\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  v = at    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\item
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%     x = vt   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\item
%\begin{equation}
%\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    a = v 1st  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\item
The acceleration is the derivative of the velocity, which is differentiated with respect of time, the partial velocity and partial time in first order ODE.
\begin{equation}
{a}= {\dot v} = \frac{\partial {v}}{\partial t}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    a = x 2nd   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\item
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    a = x/t 2nd   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\item
The acceleration is the second derivative of position, which is partial position and partial time in second order ODE:
\begin{equation}
{a} = {\ddot x} = {\frac{\partial ^{2} {x}}{\partial {t}^{2}}}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% v = x/t		 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\item
The velocity is handled similarly. It is the derivative of the position $x$ of the particle,
which is differentiated with respect of time, the partial position and partial time in first order ODE
\begin{equation}
{v} = {\dot x} ={\frac{\partial {x}}{\partial {t}}}
\end{equation}

The position x and the velocity v space is called phase space, which can be concatenated to form a 6-vector:
\begin{equation}
[ {\dot{x}_{x}},  {\dot{x}_{y}}, {\dot{x}_{z}}, {\dot{v}_{x}}, {\dot{v}_{y}}, {\dot{v}_{z}} ] = [{v}_{x}, {v}_{y}, {v}_{z}, \frac{f_x}{m}, \frac{f_y}{m}, \frac{f_z}{m}]
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  v(t+dt) = vt + (F/m) dt 	 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\item
Velocity can also be thought of as the integral of acceleration with respect of the time. If we integrate the acceleration vector over time, it gives us the new velocity. The velocity vector has been changed over this time.
\begin{equation}
v(t) = \int{a}\partial t = v(t_0) + {a}\partial t 
\end{equation}
where $v(t_0)$ is the initial velocity
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  x(t) = x(t_0) + v(t)dt   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\item
If we integrate the velocity vector over time, it gives us how the position vector changed over this time.
\begin{equation}
x(t) = \int{v(t)}\partial t = x(t_0) + v(t)\partial t 
\end{equation}
where $x(t_0)$ is the initial position
%\end{itemize}

\section{Midpoint Integrator}
Compared to the Euler method, the one-sided estimate algorithm, I introduce a more accurate and symmetric integration, centered estimate method, midpoint integrator. It computes the derivative at the center of the interval first, then computes the end of the interval.
 
%Midpoint Integration is more symmetric integration by taking midpoint of the interval of Euler Method to make the real steps of the interval.
\begin{figure*}[h]
\begin{center}
	{\label{fig:midpoint}
	 \includegraphics[width=3in]{images/midpoint.png}}
\caption{Midpoint Integrator}
\end{center}
\end{figure*}

\subsection{Midpoint Integrator Theory}

The midpoint integrator, just like others, is based on the
Taylor's series:

%\begin{eqnarray*}
$$y({t_0}+{\partial t}) = y({t_0}) + {\partial t}\dot{y_0}({t})+ \frac{{{\partial t}^2}}{2}\ddot{y_0}({t})+ O({\partial t}^3)$$

\noindent
Let's split the series into elements, which we'll later use
in a re-usable manner throughout integrator framework.

$$k_0 = y({t_0})$$
$$k_1 = {{\partial t}}\dot{y}({t}) = {{\partial t}}f(y,t)$$
$$k_2 = {\partial t}\ddot{y}({t}) = {\partial t}f(y+\frac{k_1}{2},\frac{t}{2})$$
$$y({t}+{\partial t}) = k_0 + k_2$$
where

$k_0$ is the initial state

$k_1$ is the function to find the simple Euler slope

$k_2$ is the function to find the better estimate slope at the middle of the interval

$y({t}+{\partial t})$ is the new value of a position

%\end{eqnarray*} 


%$$y({t}+{h}) = y({t}) + {h}\dot{y}({t})+ \frac{{h^2}}{2}\ddot{y}({t})+ O(h^3)$$
%$$k0 = y({t})$$
%$$k1 = {h}\dot{y}({t}) = {h}f(y,t)$$
%$$k2 = {h}\ddot{y}({t}) = {h}f(y+k1/2,t/2)$$
%$$y({t}+{h}) = k0 + k2$$


\subsection{Newton's Laws}

We apply the midpoint algorithm theory on the Newton's law in order to
achieve higher accuracy in the the relationship between the velocity and the position.
We simply plug in the elements $k_1...k_n$ into the Newton's law equation.

$$v_{k_1} = a(t)\partial t$$
$$x_{k_1} = v(t)\partial t$$
$$v_{k_2} = (v(t_0)+ \frac{v_{k_1}}{2})\partial t$$
$$x_{k_2} = (x(t_0)+ \frac{x_{k_1}}{2})\partial t$$
$$v(t) = v(t_0) + v_{k_2}\partial t$$
$$x(t) = x(t_0) + x_{k_2}\partial t$$


\section{Runge Kutta Fourth Order Integrator}

The midpoint integrator is also called Runge Kutta of Order 2 integrator because it evaluates the derivative twice. So, it is easy to explain what is Runge Kutta Fourth Order integrator. It is the integrator evaluates the derivative four times. It is the most accurate integrator compared to Euler and Midpoint. 

\begin{figure*}[h]
\begin{center}
	{\label{fig:rk4}
	 \includegraphics[width=3in]{images/rk4.png}}
\caption{Runge Kutta 4th Order Integrator}
\end{center}
\end{figure*}

\subsection{Theory}

$$y({t_0}+{\partial t}) = y({t_0}) + {\partial t}\dot{y}({t_0})+ \frac{{{\partial t}^2}}{2}\ddot{y}({t_0})+ O({\partial t}^5)$$
$$k_0 = y({t_0})$$
$${k}_{1} = {\partial t}\dot{y}({t}) = {\partial t}f(y,t)$$
$${k}_{2} = {\partial t}\ddot{y}({t}) = {\partial t}f(y+\frac{{k}_{1}}{2},\frac{t}{2})$$
$${k}_{3} = {\partial t}\ddot{y}({t}) = {\partial t}f(y+\frac{{k}_{2}}{2},\frac{t}{2})$$
$${k}_{4} = {\partial t}\ddot{y}({t}) = {\partial t}f(y+{k}_{3}, t)$$
$$y({t}+{\partial t}) = {k}_{0} + \frac{1}{6}{k}_{1} + \frac{1}{3}{k}_{2} + \frac{1}{3}{k}_{3} + \frac{1}{6}{k}_{4}$$

where

$k_0$ is the initial state

$k_1$ is the function to find the simple Euler slope

$k_2$ is the function to find the better estimate slope at the middle of the interval

$k_3$ is again to the function to find the better estimate slope at the middle of the interval

$k_4$ is the function to use excellent endpoint slope

\subsection{Newton's Laws}
$$v_{k1} = a(t)\partial t$$
$$x_{k1} = v(t)\partial t$$
$$v_{k2} = (v(t)+\frac{v_{k1}}{2})\partial t$$  
$$x_{k2} = (x(t)+\frac{x_{k1}}{2})\partial t$$
$$v_{k3} = (v(t)+\frac{v_{k2}}{2})\partial t$$  
$$x_{k3} = (x(t)+\frac{x_{k2}}{2})\partial t$$
$$v_{k4} = (v(t)+v_{k3})\partial t$$  
$$x_{k4} = (x(t)+x_{k3})\partial t$$  
$$x(t+\partial t) = x(t) + \frac{x_{k1}}{6} + \frac{x_{k2}}{3} + \frac{x_{k3}}{3} + \frac{x_{k4}}{6}$$
$$v(t+\partial t) = v(t) + \frac{v_{k1}}{6} + \frac{v_{k2}}{3} + \frac{v_{k3}}{3} + \frac{v_{k4}}{6}$$



\section{Comparison of Three Integrators}

\subsection{Efficiency} 
For a given step size, Euler is more efficient because it requires only one derivative evaluation per step, but Mid Point is about two times of computation than the Euler, and RK4 is about 4 times more inefficient than Euler.  
\begin{equation}
RK 4 = 2 \cdot Midpoint = 4 \cdot Euler 
\end{equation}
For some configuration, there may be need the Euler method because of the need of smaller simulation step. However, RK 4 will allow a much larger step size than Euler.

\subsection{Accuracy} 

If a given step size is $\partial t$, error of Euler method is $O({\partial t}^2)$ as a first-order method, error of midpoint is $O({\partial t}^3)$ (order ${\partial t}$ squared), and error of RK 4 is $O({\partial t}^5)$ 
\begin{itemize}
\item The Euler method is based on keep the first two terms of the Taylor series expansion
\begin{equation}
y({t_0}+{\partial t}) = y({t_0}) + {\partial t}\dot{y_0}({t})+O({\partial t}^2)
%y({t_0}+{\partial t}) = y({t_0}) + {\partial}\dot{y}({t})+ \frac{{{\partial t}^2}\dot{\dot{y}}({t})}{2!}+\ddots+\frac{{{\partial t}^n}\left(\frac{\partial^{n}y}{\partial{t}^n}\right)}{n!}
\end{equation}
\item An improved method which involves the second derivative is Midpoint method as following
\begin{equation}
y({t_0}+{\partial t}) = y({t_0}) + {\partial t}\dot{y_0}({t})+ \frac{{{\partial t}^2}}{2}\ddot{y_0}({t})+ O({\partial t}^3)
\end{equation}

\item An improved method which involves the four derivative is Runge Kutta method as following
\begin{equation}
y({t_0}+{\partial t}) = y({t_0}) + {\partial t}\dot{y_0}({t})+ \frac{{{\partial t}^2}}{2}\ddot{y_0}({t})+ O({\partial t}^5)
\end{equation}
\end{itemize}
\subsection{Stability} 

With smaller step time value, such as 5, the system integrated by any of the three methods is stable, not easy to explode. However, if we give the system a higher step time value, such as 50, with same mass, damping coefficient, gravity acceleration, Euler system will explode after a short period; midpoint and RK4 are more stable. 




==> dictionary.tex <==
%%
%% Appendix

%%
\addcontentsline{toc}{chapter}{Appendix}

\appendix


\chapter{Definitions and Abbreviations}

\label{appdx:defs-and-abbrs}
%\input{abbrs}

\section{Abbreviations}

\label{appdx:abbrs}

\begin{diamonds}
\item BEM - Boundary Element Method \index{BEM}%for checking collision detection
\item FEM - Finite Element Method \index{FEM}
\item FFD - Free Form Deformation \index{FFD}
\item FDM - Finite Difference Method \index{FDM}
\item ODE - Ordinary Differential Equation \index{ODE} 
\end{diamonds}

\section{Definitions}
\begin{diamonds}
\item Contact Force: when soft objects collide, they exert reaction forces
\item Contact Surface: when two soft bodies collide, the two touched surfaces
\item Elastic Object:
\item Physical Animation:
\item Real Time Animation:
\end{diamonds}

%\section{Sample Code}
%\subsection{Vector}

%\begin{figure*}[!h]
%\begin{center}
%	{\label{fig:ClassVector}
%	 \includegraphics{images/ClassVector.png}}
%\caption{Class Diagram Vector}
%\end{center}
%\end{figure*}

%%%%%%%%%%%%%%% code of the class of vector %%%%%%%%%%%%%%%%%%%%%%%%
%\begin{center}
%\begin{prog}
%\verb"class Vector{"

%\verb"public:"

%\verb"float x;                           // x-coordinate"

%\verb"float y;                           // y-coordinate"

%\verb"float z;                           // z-coordinate"

%\verb"// constructor with variables, Ax, Ay, Az, default Vector(0,0,0)"

%\verb"Vector(float Ax=0,float Ay=0,float Az=0): x(Ax),y(Ay),z(Az)"

%\verb"~Vector();"

%\verb"inline float getLength();         // get vector length"

%\verb"inline void Normalize();          // Normalize the Vector	"

%\verb"// #1 fcn - Vector addition for two vectors"

%\verb"friend Vector operator+ (const Vector & p, const Vector & q);"			

%\verb"// #2 fcn - Vector subtraction for two vectors"

%\verb"friend Vector operator- (const Vector & p, const Vector & q);"   				

%\verb"// #3 fcn - Vector multiplication"

%\verb"Vector& operator* (Vector const &);	"							

%\verb"// #3 fcn - Vector multiplication for a vector and a float	"

%\verb"Vector& operator* (float);"

%\verb"// #3 fcn - Vector multiplication for two vectors"

%\verb"friend Vector operator* (const Vector & p, const Vector & q);"

%\verb"// #4 fcn - Vector division for two vectors"

%\verb"friend Vector operator/ (const Vector & p, const Vector & q);"   				

%\verb"// #5 fcn - Vector cross product, results in a vector "

%\verb"friend Vector operator^ (Vector const &, Vector const &);	"			

%\verb"Vector& operator=(Vector const &);//#7 fcn-Vector assign operator"							

%\verb"bool operator==(Vector const &); // #8 fcn-Vector equal operator"							

%\verb"}"
%\end{prog}
%\end{minipage}
%\end{center}

%\subsection{Particle}						%%%%%%%%%%%%%%%% the class of particle %%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure*}[!h]
%\begin{center}
%	{\label{fig:ClassParticle}
%	 \includegraphics{images/ClassParticle.png}}
%\caption{Class Diagram: Partcle}
%\end{center}
%\end{figure*}

\

%\subsection{Spring}							%%%%%%%%%%%%%%%% the class of spring %%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure*}[!h]
%\begin{center}
%	{\label{fig:ClassSpring}
%	 \includegraphics{images/ClassSpring.png}}
%\caption{Class Diagram: Spring}
%\end{center}
%\end{figure*}

%\begin{center}
%\begin{minipage}{6in}
%\begin{prog}
%\verb"class Spring{"

%\verb"public:"

%\verb"Particle *sp1;             // head Particle of a Spring"

%\verb"Particle *sp2;             // tail Particle of a Spring"

%\verb"float restLen;             // lenth when Fs = 0 (Hooke force)"

%\verb"float ks;                  // Spring constant"

%\verb"float kd;                  // damping factor	"

%\verb"Vector normal;             // normal vector at the spring of a object  "

%\verb"// different types of springs to construct the object, structural,"

%\verb"// radium, shear left, and shear right"

%\verb"spring_type type;"

%\verb"// constructor with variables"

%\verb"Spring(Particle *P1, Particle *P2,float Ks=KS, float Kd=KD);"

%\verb"Spring();                      // constructor with no variable"

%\verb"~Spring();                     // destructor"

%\verb"void setRestLen();             //set the springs resting length"
	
%\verb"}"
%\end{prog}
%\end{minipage}
%\end{center}


%\subsection{Face}							%%%%%%%%%%%%%%%% the class of face %%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure*}[!h]
%\begin{center}
%	{\label{fig:ClassFace}
%	  \includegraphics{images/ClassFace.png}}
%\caption{Class Diagram: Face}
%\end{center}
%\end{figure*}

%\begin{center}
%\begin{minipage}{6in}
%\begin{prog}
%\verb"class Face{"

%\verb"public:"

%\verb"Particle *fp1;                  // first vertex "

%\verb"Particle *fp2;                  // second vertex"

%\verb"Particle *fp3;                  // third vertex"

%\verb"Spring *fs1;                    // first spring on the face "

%\verb"Spring *fs2;                    // second spring on the face"

%\verb"Spring *fs3;                    // third spring on the face "

%\verb"Vector* normal;                 // triangle normal Vector"

%\verb"// face constructor with three particles point to "

%\verb"// the three points on each face, for 2D"

%\verb"Face(Particle *Ap1, Particle *Ap2, Particle *Ap3) :"

%\verb"                      fp1(Ap1), fp2(Ap2), fp3(Ap3);"

%\verb"// face constructor with three particles point to "

%\verb"// the three points on each face, and store the spring "

%\verb"// information into the spring vector for 3D"

%\verb"Face(Particle *Ap1, Particle *Ap2, Particle *Ap3," 

%\verb"vector<Spring*> &springs):fp1(Ap1), fp2(Ap2), fp3(Ap3);"


%\verb"~Face();		                      // face destructor 	"

%\verb"// Calculate normal vector to a triangle and its field "

%\verb"void CalNormalNField(void);	 "

%\verb"}"
%\end{prog}
%\end{minipage}
%\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% object  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Object}							
%\begin{figure*}[!h]
%\begin{center}
%	{\label{fig:ClassObject}
%	 \includegraphics{images/ClassObject.png}}
%\caption{Class Diagram: Object}
%\end{center}
%\end{figure*}

\begin{center}
%\begin{minipage}{6in}
\begin{prog}
\verb"class Integrator;"

\verb"class Object{"

\verb"protected:"
	
\verb"int numParticles;           // number of particles of the object"

\verb"int numSprings;             // number of springs of the object"

\verb"Integrator* integrator;     // integrator object"

\verb"// different type of integrator, Euler, Midpoint, RK4"

\verb"integrator_type integratorType;	"

\verb"public:"

\verb"// the springs on the inner layer of the object"

\verb"vector<Spring*>  inner_springs;"

\verb"// the springs on the outer layer of the object"	

\verb"vector<Spring*>  outer_springs;"

\verb"// the particles on the inner layer of the object"
	
\verb"vector<Particle*>  inner_points;"

\verb"// the particles on the outer layer of the object"

\verb"vector<Particle*>  outer_points;"

\verb"// the surfaces on the inner layer of the object"	

\verb"vector<Face*> inner_faces; "

\verb"// the surfaces on the outer layer of the object"	

\verb"vector<Face*> outer_faces; "

\verb"// dimension type to specify the object is 1D, 2D, or 3D"	

\verb"dimensionality dim; "

\verb"// the closest point on the outer layer to mouse position"

\verb"int closest_i ; "

\verb"public:"
	
\verb"Object();                    // object constructor"
	
\verb"virtual ~Object();           // object destructor "

\verb"// get the number of particles of the object"

\verb"int GetNumberOfParticles();" 	

\verb"int GetNumberOfSprings();// get the number of springs of the object"

\verb"// choose the integrator"	

\verb"void setIntegratorType(integrator_type type);	"
	
\verb"Integrator* getIntegrator();	   // get the integrator type"
	
\verb"// update the object about forces, velocity, position"

\verb"virtual void Update(float, bool = false, float = 0, float = 0);	"		
	
\verb"	virtual void Draw() = 0;		  // display the object"

\verb"// find the closet particle on th outer layer to mouse position"

\verb"virtual void FindClosestPoint(void) ;			"

\verb"protected:"

\verb"virtual void SetParticles();  // model the particles on the object"
	
\verb"virtual void SetObject();	    // model the object"

\verb"// construct the springs to model the object"
	
\verb"virtual void Add_Structural_Spring(int, int, int);"
	
\verb"}"
\end{prog}
%\end{minipage}
\end{center}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% object 1D %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Elastic Object 1D}
\begin{figure*}[!h]
\begin{center}
	{\label{fig:ClassObject1D}
	 \includegraphics{images/ClassObject1D.png}}
\caption{Class Diagram: Object1D}
\end{center}
\end{figure*}

\begin{center}
%\begin{minipage}{6in}
\begin{prog}
\verb"class Object1D : public Object{"

\verb"public:"

\verb"Object1D();                     // object1D constructor"
	
\verb"virtual ~Object1D();            // object1D destructor"

\verb"virtual void Draw();            // display object1D"

\verb"private:	"

\verb"// model the object1D with structural spring"
	
\verb" void Add_Structural_Spring(int index, int head, int tail);"

\verb" protected:"

\verb" virtual void SetObject();     // construct the object1D"

\verb"}"
\end{prog}
%\end{minipage}
\end{center}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% object 2D %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Elastic Object 2D}
\begin{figure*}[!h]
\begin{center}
	{\label{fig:ClassObject2D}
	 \includegraphics{images/ClassObject2D.png}}
\caption{Class Diagram: Object2D}
\end{center}
\end{figure*}

\begin{center}
%\begin{minipage}{6in}
\begin{prog}
\verb"class Object2D : public Object1D{"

\verb"protected:"

\verb"// pressure at each Particles on Object2D along its normal"	

\verb"float pressure;	"

\verb"public:"

\verb"// for radium springs between two circles "

\verb"vector<Spring*>  radium_springs;"			


\verb"vector<Spring*>  shear_springs_left; // for shear spring toward left"	


\verb"vector<Spring*>  shear_springs_right;//for right spring toward right"	

\verb"Object2D();                          // constructor object2D"

\verb"virtual ~Object2D();                 // destructor object2D"

\verb"virtual void Draw();                 // display the object 2D"

\verb"inline void setPressure(float pre);  // Set Pressure  "                                                                   
\verb"inline float getPressure() ;         // Get Pressure "  

\verb"private:"
	
\verb"virtual void SetObject(void);        // model the object2D"

\verb"// model the inner or outer cirle with structural springs"	

\verb"void Add_Structural_Spring(int index, int h, int t);"	

\verb"// add the radium springs with inner point i and outer point i" 

\verb"void Add_Radium_Spring(int index);	"

\verb"//add the left shear springs with inner point i and outer point i+1"	
											
\verb"void Add_Shear_Spring(int index, int h, int t );"	

\verb"//add the right shear springs with inner point i+1 and outer point i"

\verb"// add the triangle surface to object2D"
		
\verb"virtual void Add_Faces(int i, int i1, int imid);"	

\verb"}"
\end{prog}
%\end{minipage}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% object 3D %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Elastic Object 3D}
\begin{figure*}[!h]
\begin{center}
	{\label{fig:ClassObject3D}
 \includegraphics{images/ClassObject3D.png}}
\caption{Class Diagram: Object3D}
\end{center}
\end{figure*}

\begin{center}
%\begin{minipage}{6in}
\begin{prog}
\verb"class Object3D : public Object2D{"

\verb"public:"

\verb"Object3D();             // object3D constructor"

\verb"virtual ~Object3D();    // object3D destructor"

\verb"virtual void Draw();"

\verb"void Iteration();"

\verb"void nonunitsphere();"

\verb"private:"

\verb"virtual void SetObject(void);        // model the object3D"

\verb"// model the inner or outer cirle with structural springs"

\verb"void Add_Structural_Spring(int index, int h, int t);"

\verb"// add the radium springs with inner point i and outer point i"
	
\verb"void Add_Radium_Spring(int index);"				

\verb"//add the left&right shear springs with inner point i and outer point i+1"

\verb"void Add_Shear_Spring(int index);"	

\verb"void Tetrahedron();                  // draw the single shape"

\verb"// the three points subdivide each edge on the triangle face"

\verb"Particle *pa, *pb, *pc;"	

\verb"int iterations;           // the number of iteration for subdivision"

\verb"}"
\end{prog}
%\end{minipage}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Integrator %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Integrator}
\begin{figure*}[!h]
\begin{center}
	{\label{fig:ClassIntegrator}
	 \includegraphics{images/ClassIntegrator.png}}
\caption{Class Diagram: Integrator}
\end{center}
\end{figure*}

\begin{center}
%\begin{minipage}{6in}
\begin{prog}
class Object;
\verb"class Integrator{"

\verb"protected:"
	
\verb"Object* object;"

\verb"// temp inner vector<Particle*> container for integrator computation"
	
\verb"vector<Particle*> temp_inner_points0;" 
	
\verb"vector<Particle*> temp_inner_points1;"
	
\verb"vector<Particle*> temp_inner_points2;"
	
\verb"vector<Particle*> temp_inner_points3;"
	
\verb"vector<Particle*> temp_inner_points4;"

\verb"// temp outer vector<Particle*> container for integrator computation"	

\verb"vector<Particle*> temp_outer_points0;" 
	
\verb"vector<Particle*> temp_outer_points1;"
	
\verb"vector<Particle*> temp_outer_points2;"
	
\verb"vector<Particle*> temp_outer_points3;"
	
\verb"vector<Particle*> temp_outer_points4;"

\verb"dimensionality dim;"

\verb"public:"
	
\verb"bool dragExists;		//if there is user interaction"
	
\verb"float mDragX;				// mouse position x axis"
	
\verb"float mDragY;				// mouse position y axis"
	
\verb"Integrator(Object&);//integrator constructor with the computed object"
	
\verb"virtual ~Integrator(); // integrator destructor"

\verb"//the calculation of the integration with/without external dragging force"
	
\verb"virtual void integrate(float, bool drag = false," 

\verb"               float xDrag = 0, float yDrag = 0);"

\verb"// get the object type, 1D, 2D, or 3D	"

\verb"dimensionality getDimension() {return dim;} "  

\verb"// set the object type, 1D, 2D, or 3D"

\verb"void setDimension(dimensionality dim) {this->dim = dim;}"  

\verb"protected:"
	
\verb"virtual void ExternalForces();  // accumulate gravity and dragging force"
	 
\verb"virtual void SpringForces();    // accumulate all type of springs forces "
	
\verb"virtual void PressureForces();  // accumulate pressure " 
 
\verb"virtual void AccumulateForces();// accumulate all forces acted on object" 
	
\verb"virtual void Derivatives(float, float)=0;// Differential computation"
	
\verb"virtual void CollisionDetection(int);// calculate the collision detection" 

\verb"private:"

\verb"// general spring calculation function" 
	
\verb"void CalculateSpringForces(vector<Spring *>springs,"

\verb"                      int i, bool special = false);"

\verb"}"
\end{prog}
%\end{minipage}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Euler Integrator %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Euler Method}
\begin{figure*}[!h]
\begin{center}
	{\label{fig:ClassEulerIntegrator}
	 \includegraphics{images/ClassEulerIntegrator.png}}
\caption{Class Diagram: Euler Integrator}
\end{center}
\end{figure*}

\begin{center}
%\begin{minipage}{6in}
\begin{prog}
\verb"EulerIntegrator : public Integrator{"

\verb"public:"
	
\verb"EulerIntegrator(Object&); // constructor"
	
\verb"virtual ~EulerIntegrator(); // destructor"
	
\verb"// integrate all the particles on the object"
	
\verb"virtual void Derivatives(float, float);"

\verb"protected:"
	
\verb"void k1(int, float, float);//integrate all the particles on the object"
	
\verb"void ynew(int, float, float);// get the new velocity and position"

\verb"}"
\end{prog}
%\end{minipage}
\end{center}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Midpoint Integrator %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

\subsection{Midpoint Method}
\begin{figure*}[!h]
\begin{center}
	{\label{fig:ClassMidpointIntegrator}
		 \includegraphics{images/ClassMidpointIntegrator.png}}
\caption{Class Diagram: Midpoint Integrator}
\end{center}
\end{figure*}

\begin{center}
%\begin{minipage}{6in}
\begin{prog}
\verb"class MidpointIntegrator : public EulerIntegrator{"

\verb"public:"

\verb"MidpointIntegrator(Object&);       // constructor"
	
\verb"~MidpointIntegrator();             // destructor"

\verb"protected:"

\verb"//2nd integrate to get the derivatives of velocity and position"

\verb"void k2(int, float, float);  "
	
\verb"void ynew(int, float, float);// get the new velocity and position"

\verb"}"
\end{prog}
%\end{minipage}
\end{center}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Rounga Kutta Integrator %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

\subsection{Rounge Kutta Method}
\begin{figure*}[h]
\begin{center}
	{\label{fig:ClassRungeKuttaIntegrator}
	 \includegraphics{images/ClassRungeKuttaIntegrator.png}}
\caption{Class Diagram: Rounge Kutta Integrator}
\end{center}
\end{figure*}

\begin{center}
\begin{prog}
\verb"class RungeKutta4Integrator : public MidpointIntegrator{"

\verb"public:"

\verb"RungeKutta4Integrator(Object&);     // constructor"
	
\verb"~RungeKutta4Integrator();           // destructor"

\verb"protected:"

\verb"// 3rd integrate to get the derivatives of velocity and position"

\verb"void k3(int, float, float);"
	
\verb"// 4th integrate to get the derivatives of velocity and position"
	
\verb"void k4(int, float, float);"
	
\verb"void ynew(int, float, float); //get the new velocity and position"

\verb"}"
\end{prog}
\end{center}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% View %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{View}
\begin{figure*}[!h]
\begin{center}
	{\label{fig:ClassViewSpace}
	 \includegraphics{images/ClassViewSpace.png}}
\caption{Class Diagram: View}
\end{center}
\end{figure*}

\begin{center}
\begin{prog}
\verb"Object1D object1D;      // initial the object1D"

\verb"Object2D object2D;      // initial the object2D"

\verb"Object3D object3D;      // initial the object3D"

\verb"class ViewSpace{"

\verb"public:"

\verb"ViewSpace();            // constructor"

\verb"~ViewSpace();           // destructor"

\verb"Draw();                 // draw object and environment"

\verb"Update();               // update the integrator"

\verb"}"
\end{prog}
\end{center}
  



==> difficulties.tex <==

\clearpage
\section{Difficulties}
\thispagestyle{plain}

-	implement self-intersection check and resolution
-	if the particles are non-neighboring, it is difficult to prevent them from intersecting one another

Gas:
-	we have a gas inside of the body
-	we are only about macroscopic, not care about micro-collisions
-	we can use ideal gas approximation


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> index.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\addcontentsline{toc}{chapter}{Index}
\printindex

==> mathematics.tex <==
\chapter{Math Methodology}
\label{chapt:physical based numerical integration methodology}
\index{Physical Based Numerical Integration Methodology}


A one-dimensional object model includes gravity force ${\bf F}^{g}$, user applied force ${\bf F}^{a}$, and collision force ${\bf F}^{c}$ as external forces; linear structural spring force ${\bf F}^{h}$ and spring damping force ${\bf F}^{d}$ as internal forces.

\begin{equation}
{\bf F} = {\bf F}^{g} + {\bf F}^{h} + {\bf F}^{d} + {\bf F}^{a} + {\bf F}^{c}
\end{equation}

A two-dimensional object model is considered as a closed shape with air pressure inside. Then, the air pressure ${\bf F}^{p}$ is a new internal force exist in two-dimensional object in addition to the common forces we have already discussed in one-dimensional object. Accumulation of forces on a three-dimensional object particle are similar to forces applied on the two-dimensional one. The only difference is that all forces on three-dimensional objects are extended to axis z.

\begin{equation}
{\bf F} = {\bf F}^{g} + {\bf F}^{h} + {\bf F}^{d} + {\bf F}^{a} + {\bf F}^{c} + {\bf F}^{p}
\end{equation}

\section{Gravity Force} 
Gravity force is a constant force at which the earth attracts objects based on their masses. In most cases, the particle system does not include gravitation, but, in my system, particle gravities represent object's density. User can set particle gravities to a non-zero value. ${\bf g}$ is a constant vector of the gravitational field which points to opposite of y axis. 

\begin{equation}
{\bf F}^{g}= m{\bf g}
\end{equation}

A gravitational force for a one-dimensional or two-dimensional object is
\[{\bf F}^{g}=
\left[\begin{array}{c}
{0} \\
{-m{\bf g}} \end{array}\right]\]

A gravitational force for a three-dimensional object is
\[{\bf F}^{g}=
\left[\begin{array}{c}
{0} \\
{-m{\bf g}} \\
{0} \end{array}\right]\]



\section{Spring Hooke's Force} 
Spring force is a linear force exerted by a compressed or 
stretched spring upon two connected particles. The particles 
which compress or stretch a spring are always acted upon 
by this spring force which restores them to their 
equilibrium positions. It is calculated as following according 
to Hooke's law, which describes the opposing force exerted by a spring.

\begin{equation}
{\bf F}_{12}^{h} = -\left(|{\bf r}_{2}-{\bf r}_{1}|-r_{l}\right)\cdot{k}_{s}
\end{equation}

\noindent
where 

\noindent
${\bf r}_{1}$ is the first particle position,

\noindent
${\bf r}_{2}$ is the second particle position, 

\noindent
${r}_{l}$ is default length of the  resting spring between the two particles,

\noindent
${k}_{s}$ is the stiffness of the spring,

\noindent 
when $|{\bf r}_{2}-{\bf r}_{1}|-r_{l}=0$, the spring is resting,

\noindent
when $|{\bf r}_{2}- {\bf r}_{1}|-r_{l}>0$, the spring is extending,

\noindent
when $|{\bf r}_{2}-{\bf r}_{1}|-r_{l}<0$, the spring is contracting.



\section{Spring Damping Force} 
Spring damping force is also called viscous damping. It is opposite force of the hook spring force in order to simulate the natural damping and resist the motion. It is also opposite to the velocity of the moving mass particle and is proportional to the velocity because the spring is not completely elastic and it absorbs some of the energy and tends to decrease the velocity of the mass particle attached to it. It is needed to simulate the natural damping due to the forces of friction. More importantly, it is useful to enhance numerical stability and is required for the model to be physically correct\cite{brar97}. 

a force with magnitude proportional to that of the velocity of the object but opposite in direction to it. 
\begin{equation}
{\bf F}_{12}^{d} = 
\left({\bf v}_{2}-{\bf v}_{1}\right)\cdot
\left(\frac{{\bf r}_{2}-{\bf r}_{1}}{|{\bf r}_{2}-{\bf r}_1|}\right)
\cdot{k}_{d}
\end{equation}
\noindent
where

\noindent
$\left(\frac{{\bf r}_{2}-{\bf r}_{1}}{|{\bf r}_{2}-{\bf r}_1|}\right)$ is the normal vector of spring,

\noindent
${\bf v}_{1}$ and ${\bf v}_{2}$ is the velocity of the two masses,

\noindent
${k}_{d}$ is spring damping coefficient, 

\noindent
when the two endpoints moving away from each other, 

\noindent
the force imparted from the damper will act against that motion,

\noindent
when the two endpoints moving toward each other, 

\noindent
the damper will act against the squeeze motion. 

\section{Mouse Drag Force} is the force when user interacts with the elastic object through mouse. If one particle on the object is dragged, the dragging force for rest particles are passed through by springs. 

We can consider one end of the string connects to the mouse position and the other end of the string connects to the nearest particle on the object. This string is elastic, so it has all the spring's properties, such as hook spring force and damping force. This is s momentary force for interacting with the simulation and should subtract that force from the sum of the accumulated force. The mouse dragging force can be presented as following: 

\begin{equation}
{\bf F}^{m}=\left(|\vec{r}_{m}-\vec{r}_{i}|-r_{lm}\right)\cdot{k}_{sm}+ \left(\vec{v}_{m}-\vec{v}_{i}\right)\cdot\left(\frac{\vec{r}_{m}-\vec{r}_{i}}{|\vec{r}_{m}-\vec{r}_{i}|}\right)\cdot{k}_{dm}
\end{equation}

where

$\vec{r}_{m}$ is the mouse position,

$\vec{r}_{i}$ is the particle position nearest to mouse, 

$\vec{r}_{lm}$ is default length of the  resting mouse spring,

${k}_{sm}$ is the stiffness of the mouse spring,

$\vec{v}_{m}$ is the velocity of the mouse represented as a mass 

$\vec{v}_{i}$ is the mass for the nearest particle,

${k}_{dm}$ is spring damping coefficient for the mouse spring 
 

\section{Collision Force}

If an object continues traveling under a force without colliding with other objects, it will be very difficult to describe objects motion and elastic response in reality. There are two steps to describe the collision effects: test the elastic object if particles hit anything; adjust position by computing the impulse.

\paragraph*{Collision Detection} is a geometric problem of determining if a moving object intersected with other objects at some point between an initial and final configuration. In our elastic object simulation system, we are concerned with the problem of determining if particles collide with solid planes. 

We take one particle shown in Fig.(\ref{fig:collision}) as an example:

\begin{figure*}[h]
\begin{center}
	{\label{fig:collision}
	 \includegraphics[width=2in]{images/collision.png}}
\caption{Particle Collision and Impact}
\end{center}
\end{figure*}

\begin{equation}
P(x,y,z) = ax +by + cz + d = 0
\end{equation}

if $F(x,y,z)>0$, the particle is on one side of the plane,

if $F(x,y,z)<0$, the particle is on the other side of the plane.

can check all the vertices for the condition.

At each time step, looping through all the particles on the object, each particle is checked if it is outside of the interacting plane. When the particle $i$ collides with the plane, an artificial collision spring, which has elasticity and damping properties as an ordinary spring, is generated between this particle and the plane. This artificial collision spring will push the colliding particle backward according to the normal force, then all the other particles will be applied with this new distortion force. Eventually, the elastic object will stop its motion because of friction loss is calculated. This is the simplest case of collision detection.

%A particle can be treated as a line segment from its previous position to its current position:
If we are colliding against static objects, then we
just need to test if the line segment intersects
the object.
Colliding against moving objects requires some
additional modifications that we will also look at.

The normal force is the support force exerted upon an object which is in contact with another stable object. For example, if a book is resting upon a surface, then the surface is exerting an upward force upon the book in order to support the weight of the book. On occasions, a normal force is exerted horizontally between two objects which are in contact with each other.

The friction force is the force exerted by a surface as an object moves across it or makes an effort to move across it. The friction force opposes the motion of the object. For example, if a book moves across the surface of a desk, then the desk exerts a friction force in the opposite direction of its motion. Friction results from the two surfaces being pressed together closely, causing intermolecular attractive forces between molecules of different surfaces. As such, friction depends upon the nature of the two surfaces and upon the degree to which they are pressed together. The friction force can be calculated using the equation:

%$F_friction = \mu F_{Normal}$ where $\mu$ is the friction coefficient


 
 
General goals: given two objects with current
and previous orientations specified, determine if,
where, and when the two objects intersect
- Alternative: given two objects with only current
orientations, determine if they intersect
- Sometimes, we need to find all intersections.
Other times, we just want the first one.
Sometimes, we just need to know if the two
%objects intersect and dont need the actual intersection data.

\paragraph*{Collision Response} is a physics
problem of determining the impulses of the collision.


is the force to make object bounce away from the fixed interacting plane when elastic object collision happens. Some energy is lost in the collision response as described in the penalty method. The inclined plane is 


Penalty Method

When collision happens, must perform some action to prevent the object penetrating even deeper. Object should bounce away from the colliding object. Some energy is usually lost during collision. Several ways to handle collision response, we will use the penalty method.

When collision happens, put an artificial collision spring at the point of collision, which will push the object backwards and away from the colliding object. Collision springs have elasticity and damping, just like ordinary springs. 

e: elasticity of the collision (usually [0.0..1.0])
f: friction (sliding friction, if you want)
N: plane normal
V0: initial projectile velocity
V1: final projectile velocity
subscript (n): component parallel to n
subscript (p): component perpendicular to n

V0n = V0.projectOn(N)
V0p = V0 - V0n
V1 = -V0n*e + V0p*f
if no sliding friction:
V1 = -V0n*e + V0p*e = (-V0n + V0p)*e

In this two-dimensional method, the particles on the outer layer still follow the same method and same pre-defined boundary. However, for the particles on the inner layer, the boundary is constrained to the outer layer instead of the wall and floor. 



\paragraph*{Spring Hook's Force and Damping Force} have been discussed as the type of structural spring in one-dimensional object. Here, the same method applies on the other three types of spring, such as radium springs, shear left springs, and shear right springs with different spring stiffness and spring damping factor. So, the total hook spring force and spring damping force for each spring, or more accurate saying, on each particle is:

\begin{eqnarray*}
\vec{F}^{total spring} = {F}_{structure}^{h} + {F}_{structure}^{d} + {F}_{radium}^{h} + {F}_{radium}^{d}\\
 											 + {F}_{shear left}^{h} + {F}_{shear left}^{d} + {F}_{shear right}^{h} + {F}_{shear right}^{d}
\end{eqnarray*}
\paragraph*{Mouse Drag Force} is only applied on the outer circle of the double layered object when user interacts the object with mouse. The nearest particle from the outer layer to the mouse position is found when mouse is pressed, and the dragging force for rest of particles on inner layer and outer layer are passed through by the four different types of springs. 

\section{Normal Force}
\subsection{2D Normals} are unit vectors perpendicular to specified data structure, such as vertex, line, and polygonal facets. They are used in rendering scenes techniques to calculate the light sources are reflected to the camera view. Normal calculation is also useful in mapping texture techniques. 
 
\begin{itemize}
\item particle normal: is the average of the normals of the subtended neighboring particles. To calculate the particle normal is to add the normals for each face adjoining the particle, and then normalizing the sum.

\item spring normal: is based on the two particles  $P_1, P_2$ connected on the spring. It is perpendicular to the spring itself.

\item face normal: is perpendicular to its surface based on the any pair of springs on the surface. The normal for a triangle surface composed with three particles $P_1, P_2, P_3$ is computed as the cross product of the springs $P_2-P_1$ and $P_2-P_3$.
\end{itemize}

However, the usage of normal calculation method in my elastic object simulation system is for analyzation of the direction of the pressure force inside of the object. Only spring normal is calculated here because all the internal and external forces will apply on each spring, and the spring will define the particles' force who connect onto it. 

For the single spring $Spring_{12}$, the coordinates for particle $P_1$ is $(x_1, y_1)$; the coordinates for particle $P_2$ is $(x_2, y_2)$. The normal to this spring is the spring rotate  $90^0$ at axis z according to the space position. So, we can get the coordinates of the normal in x axis and y axis as following

\[\left[\begin{array}{c}
{x'} \\
{y'} \end{array}\right]= \left[\begin{array}{cc} 
cos{90^{0}} & -sin{90^{0}} \\
sin{90^{0}} & cos{90^{0}} \end{array} \right]
\left[\begin{array}{c} 
{x_2-x_1} \\
{y_2-y_1} \end{array} \right]\]

\[\left[\begin{array}{c}
{x'} \\
{y'} \end{array}\right]= \left[\begin{array}{c}
-\left({y_2-y_1}\right)\\
{x_2-x_1} \end{array} \right]\]

\subsection{3D Normals} are as important as the role in two-dimensional object simulation. The calculation is important because it will define the direction of the internal air pressure force, either compress the elastic object or expand its volume. In three-dimensional simulation, the normal of a spring in the space position can be represent as
 
\[\left[\begin{array}{c}
{x'} \\
{y'} \\
{z'} \\
{1} \end{array}\right]= 
\left[\begin{array}{cccc} 
cos{90^{0}} & -sin{90^{0}} & 0 & 0 \\
sin{90^{0}} & cos{90^{0}} & 0 & 0\\
0 & 0 & 1 & 0 \\
0 & 0 & 0 & 1 \end{array} \right]
\left[\begin{array}{cccc} 
1 & 0 & 0 & 0 \\
0 & cos{90^{0}} & sin{90^{0}} & 0 \\
0 & -sin{90^{0}} & cos{90^{0}} & 0 \\
0 & 0 & 0 & 1 \end{array} \right]\]
\[\left[\begin{array}{cccc} 
cos{90^{0}} & 0 & -sin{90^{0}} & 0 \\
0 & 1 & 0 & 0 \\
sin{90^{0}} & 0 & cos{90^{0}} & 0\\
0 & 0 & 0 & 1 \end{array} \right]
\left[\begin{array}{c} 
{x_2-x_1} \\
{y_2-y_1} \\
{z_2-z_1} \\
{1} \end{array} \right]\]

Therefore,

\[\left[\begin{array}{c}
{x'} \\
{y'} \\
{z'} \\
{1} \end{array}\right]= \left[\begin{array}{c}
-\left({x_2-x_1}\right)\\
{z_2-z_1} \\
{y_2-y_1} \\
{1} \end{array} \right]\]



\section{Air Pressure Force}
In order to describe an elastic object more accurately, especially soft body of human beings and animals, the calculation only about the elastic force on the object's surface is not enough. There must be the flow force inside of the elastic object to make the object oscillately and wobbly looking when it is deformed. The internal force will be applied on one direction and relieved in another direction.  

The pressure force, which is parallel to the normal vector of the surface, will be calculated for every spring, then update each particle's direction. The pressure vector is always acting in a direction of normal vectors to the surface, so the shape will not deform completely. If only pressure system without mass-spring system, the object will get explode.

\begin{figure*}[h]
\begin{center}
	\subfigure[The External Gravity Force Is Applied Producing A Pressure Wave]
	{\label{fig:TwoD3}
 		\includegraphics[width=2in]{images/TwoD3.png}}
 		\hspace{.6in}
	\subfigure[The Object Restores Its Shape With Internal Air Pressure Force]
	{\label{fig:TwoD2}
 		\includegraphics[width=2in]{images/TwoD2.png}}
\caption{Double-layered Two-dimensional Elastic Object filled With Air}
\end{center}
\end{figure*}

In the figure a, the object is deformed from bottom because of the gravity force. If there is no internal air pressure, the object will collapse unless the springs are hard enough to avoid the failure. With the very hard springs, it is difficult to simulate the reality of the elasticity. The real elastic object will squish outwards to restore its shape as described in figure b.  
 
The simplified version of the Ideal Gas Law\cite{mm04}, also known as Clausius Clapeyron Equation, is used to describe such effect:
 
\begin{equation}
\vec{P}V = P\cdot\vec{n}RT \iff \vec{P} = \frac{P\cdot\vec{n}RT}{V}
\end{equation}
where

$\vec{P}$ is the pressure force vector,

$P$ is the pressure value, 

$V$ is the volume of the object, 

$\vec{n}$ is the normal vector to the edges on the object, 

$R$ is the gas constant, 

$T$ is the gas temperature. 

In order to find an estimate pressure inside of the object which will be applied to particles later, we need to calculate the volume of the object. The approximation of the volume calculation is considered to be enough because we only care about the volume in general change. 

To calculate the object volume, we use Gauss Theorem for closed shape object. It replaces the integration over the volume by integration of the surface. The simplified integration of body volume is introduced by Maciej Matyka \cite{mm04}:

\begin{equation}
V = \displaystyle\sum_{i=0}^{i=NUMS-1}\frac{1}{2}|x_{1}-x_{2}|\cdot \vec{n}\cdot length
\end{equation}

where

$V$ is the volume of the object, 

$|x_{1}-x_{2}|$ is the absolute difference of the spring of the start and end particles at axis x,

$\vec{n}$ is the normal vector to this spring at axis x,

$length$ is the spring's length.

The internal air pressure force prevents the object from collapsing when it is compressed by external forces. Moreover, it simulates the object in reality by demonstrating the derivate calculation of the force and volume.  


\section{Algorithm}

\begin{itemize}
\item Step 9: Split object into regions, integrate density and weight in each region to modify mass. The current system considers the particle weights are all same. In the future model, the density and weight of the particles can be vary in order to get the non-unit motion.
\item Step 10: Changing the spring constants for the different types of springs of the system. Also, different density effects can be realized. The consequence is that the force of each particle varies from the different compression of springs.
\item Step 11: Initialize density as gas, liquid, or rubber inside of the body and introduce some simple physics to describe it. In the current system, only air pressure material is considered and only pressure equation will be used for this extra force computation.
\item Step 12: Calculate all forces accumulated on the each inner and outer layer particle except air pressure force. 
\item Step 13: Calculate volume of the inner layer of the elastic object. 
\item Step 14: Calculate volume of the outer layer of the elastic object. 
\item Step 15: Calculate the normal of springs on each triangular face to define the pressure force direction.
\item Step 16: Calculate the force from the internal air pressure by multiplying the result by field of the face.
\item Step 17: Accumulate finally pressure force to each particle.
\item Step 18: Integration the object's momentum motion by calculating the derivative velocity and its new position for each particle.
\item Step 19: Resolve collision detection and response and define the updated position.
\item Step 20: Loop through Step 12.  
\end{itemize}

==> methodology.tex <==
\chapter{Soft Body Modeling Methodology}
\label{chapt:soft body modeling methodology}
\index{Soft Body Modeling Methodology}

In this chapter, I will introduce the methodology of modeling an elastic object. Here, let's have a look at the basic data structure.
 
\paragraph*{Particles} are the objects that have mass, position, velocity, normals, and forces applied on them, but have no spatial extent. Moreover, the differential position and velocity change, are also two properties for these computation of each particle.
\paragraph*{Springs} are massless with natural length non equal to zero. They are the linkage of particles. There must be at least one spring connects with two particles. The normal for a spring is perpendicular to the spring.
\paragraph*{Faces} are the data type consists of springs as the edge and particles as the corners. The normal for a face is the cross product of the any two spring edges of the face.



\section{1D}
The techniques used in one-dimensional object are present here, which are applied subsequently to models in two and three dimensions. One end of the spring is fixed on the ceiling. User interacts with the other end of the spring by dragging it or squeeze it. The force of a single spring is restricted to one dimensional. The dangling end strives apart at certain distance from the fixed end because spring generates opposite force when pulled apart or pushed together along with a spring damping term which models the loss energy. A rubber rope is a good example of 1D elastic objects.\cite{go01}

\subsection{Geometric Modeling}
\paragraph*{Particle} There are two mass particles on a single spring.  
\paragraph*{Spring} In one-dimensional object, only one type of the spring, structural spring, is introduced. Structural spring, is used to model the object shape, connected by the two mass particles in this case.

\begin{figure*}[h]
\begin{center}
	\subfigure[The initial spring system is at rest]
	{\label{fig:OneD1}
	 \includegraphics[width=2in]{images/OneD1.png}}
	 \hspace{.6in}
	\subfigure[The squeeze force is applied]
  {\label{fig:OneD2}
	 \includegraphics[width=2in]{images/OneD2.png}}
\caption{One Dimensional Elastic Object}
\end{center}
\end{figure*}

In figure a, the spring is at the initial state of equilibrium. The length of the natural spring is $l$ and the force $f$ is zero. In figure b, the spring is squeezed. The current spring length $l'<l$ and the force of the spring is pushed out, which is larger than zero. When the spring is stretched out, the current spring length $l'>l$ and the force of the spring is held back, which is less than zero. 
\subsection{Algorithm}
\begin{itemize}
\item Step 1: Create two particles with mass value $m_{\left( x, y \right)}$, the position $\vec{r}_{\left(x, y\right)}$, velocity $\vec{v}_{\left(x,y\right)}$. 
\item Step 2: $Mass_{1}$ is fixed, so its gravity force can be considered as 0. $Mass_{2}$ is connected with a spring, and its gravity force is $\vec{F}^{g}$.
\item Step 3: Calculate all forces accumulated on the first mass particle, and calculate all the forces accumulated on the second mass particle.
\item Step 4: Integration the object's motion by calculating the derivative velocity and its new position for each particle.
\item Step 5: Loop through Step 3.  
\end{itemize}

\subsection{Forces}

For this one dimensional object model, it includes the gravity force $\vec{F}^{g}$, the mouse dragging force $\vec{F}^{m}$, and collision force $\vec{F}^{c}$ as external force; linear structural spring force $\vec{F}^{h}$ and spring damping force $\vec{F}^{d}$ as internal force.

\begin{equation}
\vec{F} = \vec{F}^{g} + \vec{F}^{h} + \vec{F}^{d} + \vec{F}^{m} + \vec{F}^{c}
\end{equation}

\paragraph*{Gravity Force} is the constant force based on the mass. Here, $\vec{g}$ is a constant vector of the gravitational field, pointing down. In most case, the particle system does not include gravitation, but, in my system, user can set the particle gravity more than 0.

\begin{equation}
\vec{F}^{g}=m\vec{g}
\end{equation}

\paragraph*{Spring Hook's Force} is the linear spring force appears between two connected particles. It is calculated as following according to Hooke's law,

\begin{equation}
\vec{F}_{12}^{h} = \left(|\vec{r}_{1}-\vec{r}_{2}|-r_{l}\right)\cdot{k}_{s}
\end{equation}

where 

$\vec{r}_{1}$ is the first particle position,

$\vec{r}_{2}$ is the second particle position, 

$\vec{r}_{l}$ is default length of the  resting spring between the two particles,

${k}_{s}$ is the stiffness of the spring,
 
when $|\vec{r}_{1}-\vec{r}_{2}|-r_{l}=0$, the spring is resting,

when $|\vec{r}_{1}-\vec{r}_{2}|-r_{l}>0$, the spring is extending,

when $|\vec{r}_{1}-\vec{r}_{2}|-r_{l}<0$, the spring is contracting.

\paragraph*{Spring Damping Force} is also called viscous damping. It is opposite force of the hook spring force in order to simulate the natural damping and resist the motion. It is also opposite to the velocity of the moving mass particle and is proportional to the velocity because the spring is not completely elastic and it absorbs some of the energy and tends to decrease the velocity of the mass particle attached to it. It is needed to simulate the natural damping due to the forces of friction. Moreover, it is useful to enhance numerical stability and is required for the model to be physically correct\cite{brar97}. 

\begin{equation}
\vec{F}_{12}^{d} = \left(\vec{v}_{1}-\vec{v}_{2}\right)\cdot\left(\frac{\vec{r}_{1}-\vec{r}_{2}}{|\vec{r}_{1}-\vec{r}_2|}\right)\cdot{k}_{d}
\end{equation}

where

$\left(\frac{\vec{r}_{1}-\vec{r}_{2}}{|\vec{r}_{1}-\vec{r}_2|}\right)$ is the normal vector of spring,

$\vec{v}_{1}$ and $\vec{v}_{2}$ is the velocity of the two masses,

${k}_{d}$ is spring damping coefficient, 

when the two endpoints moving away from each other, 

the force imparted from the damper will act against that motion,

when the two endpoints moving toward each other, 

the damper will act against the squeeze motion. 

\paragraph*{Mouse Drag Force} is the force when user interacts with the elastic object through mouse. If one particle on the object is dragged, the dragging force for rest particles are passed through by springs. 

We can consider one end of the string connects to the mouse position and the other end of the string connects to the nearest particle on the object. This string is elastic, so it has all the spring's properties, such as hook spring force and damping force. This is s momentary force for interacting with the simulation and should subtract that force from the sum of the accumulated force. The mouse dragging force can be presented as following: 

\begin{equation}
\vec{F}^{m}=\left(|\vec{r}_{m}-\vec{r}_{i}|-r_{lm}\right)\cdot{k}_{sm}+ \left(\vec{v}_{m}-\vec{v}_{i}\right)\cdot\left(\frac{\vec{r}_{m}-\vec{r}_{i}}{|\vec{r}_{m}-\vec{r}_{i}|}\right)\cdot{k}_{dm}
\end{equation}

where

$\vec{r}_{m}$ is the mouse position,

$\vec{r}_{i}$ is the particle position nearest to mouse, 

$\vec{r}_{lm}$ is default length of the  resting mouse spring,

${k}_{sm}$ is the stiffness of the mouse spring,

$\vec{v}_{m}$ is the velocity of the mouse represented as a mass 

$\vec{v}_{i}$ is the mass for the nearest particle,

${k}_{dm}$ is spring damping coefficient for the mouse spring 
 

\paragraph *{Collision Force} is the force to make object bounce away from the fixed interacting plane when elastic object collision happens. Some energy is lost in the collision response as described in the penalty method. The inclined plane is 

\begin{equation}
F(x,y,z) = ax +by + cz + d = 0
\end{equation}

if $F(x,u,z)>0$, the particle is on one side of the plane,

if $F(x,u,z)<0$, the particle is on the other side of the plane.

At each time step, looping through all the particles on the object, each particle is checked if it is outside of the interacting plane. When the particle $i$ collides with the plane, an artificial collision spring, which has elasticity and damping properties as an ordinary spring, is generated between this particle and the plane. This artificial collision spring will push the colliding particle backward according to the normal force, then all the other particles will be applied with this new distortion force. Eventually, the elastic object will stop its motion because of friction loss is calculated. This is the simplest case of collision detection.

\subsection{Result and Summary}
I have modeled a one-dimensional elastic object with one spring connected by two particles. Furthermore, I have illustrated the basic algorithm to model a simple elastic object and introduced associated forces to simulate this elastic object.

\section{2D}
In this section, I extend the one-dimensional elastic object to two dimensions. I create two separated elastic circles, inner circle and outer circle. Both of them consist of the same modeling structure as one-dimensional, mass particles  and springs. Then, the two concentric circles, inner and outer, are connected by various springs to become one two-layered elastic object. However, the distinct features in two-dimensional object are more types of springs presented and the air pressure inside the two-layer close shape is calculated. The spring surface prevents infinite expansion of the air; meanwhile the internal pressure avoids the surface collapsing.

\subsection{Geometric Modeling}

Two-dimensional object is made of three types of primitives, mass particles, springs, and indexed triangles faces. 

\paragraph*{Particles} are defined based on their coordinates at axis x and y in the space position. Let's take a circle with twelve particles as an example. The space position for each particle is 

\begin{equation}
x = Radius \cdot \cos \left( \frac{i \cdot 2 \cdot \pi}{numParticles} \right)
\end{equation}
\begin{equation}
y = Radius \cdot \sin \left( \frac{i \cdot2  \cdot \pi}{numParticles} \right)
\end{equation}

\begin{figure*}[h]
\begin{center}
	{\label{fig:TwoD11}
	 \includegraphics[width=2in]{images/TwoD11.png}}
\caption{Two-dimensional Elastic Object with Single Layer}
\end{center}
\end{figure*}

\paragraph*{Springs} Except the structural spring, which also exists in one-dimensional object, there are another two types of springs, radium spring and shear spring.

\begin{diamonds}
\item	Structural springs: give the basic structure of inner circle and outer circle to prevent neighboring particles from getting too close to one another (draw in red color). 

Linkage of each structural spring i is to connect with two particles${P}_{i}$ and ${P}_{i+1}$ or ${P}_{i-1}$ and ${P}_{i}$.

\item Radium springs: are the springs connected from particles on inner circle to the particle on the outer circle as part of the circle radium n order to prevent the bending of the surface (draw in green color).

Linkage of each radium spring i is to connect with particle ${P}^{inner}_{i}$ and the particle ${P}^{outer}_{i}$. 

\item Shear springs: are springs connect from particles on inner circle to their diagonal neighbors on outer circle in order to avoid the surface fold over (draw in pink color).

Linkage of each left shear spring i is to connect with particle ${P}^{outer}_{i}$ diagonally and the particle ${P}^{inner}_{i-1}$; connect with particle ${P}^{outer}_{i+1}$ diagonally and the particle ${P}^{inner}_{i}$ and so or.

Linkage of each right shear spring i is to connect with particle ${P}^{outer}_{i-1}$ diagonally and the particle ${P}^{inner}_{i}$; connect with particle ${P}^{outer}_{i}$ diagonally and the particle ${P}^{inner}_{i+1}$ and so or.
\end{diamonds} 

\begin{figure*}[h]
\begin{center}
	{\label{fig:TwoD111}
 		\includegraphics[width=2in]{images/TwoD111.png}}
\caption{Three Types of Springs on a Two-dimensional Object}
\end{center}
\end{figure*}

\paragraph*{Faces} are the data structure for the only purpose of drawing and displaying a filled object to a two-dimensional object. The triangular facets can be drawn separately and  visualized as a filled circle. 
  
\begin{figure*}[h]
\begin{center}
	{\label{fig:TwoD1} \includegraphics[width=2in]{images/TwoD1.png}}
\caption{Two-dimensional Elastic Object Facets}
\end{center}
\end{figure*} 
 
\paragraph*{Normals} are unit vectors perpendicular to specified data structure, such as vertex, line, and polygonal facets. They are used in rendering scenes techniques to calculate the light sources are reflected to the camera view. Normal calculation is also useful in mapping texture techniques. 
 
\begin{itemize}
\item particle normal: is the average of the normals of the subtended neighboring particles. To calculate the particle normal is to add the normals for each face adjoining the particle, and then normalizing the sum.

\item spring normal: is based on the two particles  $P_1, P_2$ connected on the spring. It is perpendicular to the spring itself.

\item face normal: is perpendicular to its surface based on the any pair of springs on the surface. The normal for a triangle surface composed with three particles $P_1, P_2, P_3$ is computed as the cross product of the springs $P_2-P_1$ and $P_2-P_3$.
\end{itemize}

However, the usage of normal calculation method in my elastic object simulation system is for analyzation of the direction of the pressure force inside of the object. Only spring normal is calculated here because all the internal and external forces will apply on each spring, and the spring will define the particles' force who connect onto it. 

For the single spring $Spring_{12}$, the coordinates for particle $P_1$ is $(x_1, y_1)$; the coordinates for particle $P_2$ is $(x_2, y_2)$. The normal to this spring is the spring rotate  $90^0$ at axis z according to the space position. So, we can get the coordinates of the normal in x axis and y axis as following

\[\left[\begin{array}{c}
{x'} \\
{y'} \end{array}\right]= \left[\begin{array}{cc} 
cos{90} & -sin{90} \\
sin{90} & cos{90} \end{array} \right]
\left[\begin{array}{c} 
{x_2-x_1} \\
{y_2-y_1} \end{array} \right]\]

\[\left[\begin{array}{c}
{x'} \\
{y'} \end{array}\right]= \left[\begin{array}{c}
-\left({y_2-y_1}\right)\\
{x_2-x_1} \end{array} \right]\]


\subsection{Algorithm}

\begin{itemize}
\item	Step 1: Define a group of particles' position to make a inner circle with mass value $m_{\left( x, y \right)}$, the position $\vec{r}_{\left(x, y\right)}$, velocity $\vec{v}_{\left(x,y\right)}$.
\item Step 2: All the particles have the default gravity force $\vec{F}^{g}$.
\item Step 3: Add the structural springs to the inner circle.
\item Step 4: Repeat Step 1 to 3 to create an outer circle two times bigger than the inner circle.
\item Step 5: Loop through the number of structural springs to add the same number of radium springs according to the linkage of the inner and outer particles.
\item Step 6: Loop through the number of structural springs to add the same number of shear left springs and shear right springs according to the linkage of the inner and outer particles.  
\item Step 7: Calculate all forces accumulated on the each particle.
\item Step 8: Integration the object's motion by calculating the derivative velocity and its new position for each particle.
\item Step 9: Loop through Step 7.  
\end{itemize}

\subsection{Forces}
For this two dimensional object model, we can consider it as a closed shape of 2D elastic cloth with air pressure inside. So, the air pressure $\vec{F}^{p}$ is the new force exist in two-dimensional object additional to the common forces we have already talked about in one-dimensional object, such as the gravity force $\vec{F}^{g}$, the mouse dragging force $\vec{F}^{m}$, and collision force $\vec{F}^{c}$ as external force; linear structural spring force $\vec{F}^{h}$ and spring damping force $\vec{F}^{d}$ as internal force.

\begin{equation}
\vec{F} = \vec{F}^{g} + \vec{F}^{h} + \vec{F}^{d} + \vec{F}^{m} + \vec{F}^{c} + \vec{F}^{p}
\end{equation}

\paragraph*{Gravity Force} for each particle is exactly same as the gravity force for the particle of one dimensional model. Loop through the number of the particles, and set the gravity force to $(0, m\vec{g})$, which points to opposite of y axis.

\paragraph*{Spring Hook's Force and Damping Force} have been discussed as the type of structural spring in one-dimensional object. Here, the same method applies on the other three types of spring, such as radium springs, shear left springs, and shear right springs with different spring stiffness and spring damping factor. So, the total hook spring force and spring damping force for each spring, or more accurate saying, on each particle is:

\begin{eqnarray*}
\vec{F}^{total spring} = {F}_{structure}^{h} + {F}_{structure}^{d} + {F}_{radium}^{h} + {F}_{radium}^{d}\\
 											 + {F}_{shear left}^{h} + {F}_{shear left}^{d} + {F}_{shear right}^{h} + {F}_{shear right}^{d}
\end{eqnarray*}
\paragraph*{Mouse Drag Force} is only applied on the outer circle of the double layered object when user interacts the object with mouse. The nearest particle from the outer layer to the mouse position is found when mouse is pressed, and the dragging force for rest of particles on inner layer and outer layer are passed through by the four different types of springs. 

\paragraph*{Air Pressure Force}
In order to describe an elastic object more accurately, especially soft body of human beings and animals, the calculation only about the elastic force on the object's surface is not enough. There must be the flow force inside of the elastic object to make the object oscillately and wobbly looking when it is deformed. The internal force will be applied on one direction and relieved in another direction.  

The pressure force, which is parallel to the normal vector of the surface, will be calculated for every spring, then update each particle's direction. The pressure vector is always acting in a direction of normal vectors to the surface, so the shape will not deform completely. If only pressure system without mass-spring system, the object will get explode.

\begin{figure*}[h]
\begin{center}
	\subfigure[The External Gravity Force Is Applied Producing A Pressure Wave]
	{\label{fig:TwoD3}
 		\includegraphics[width=2in]{images/TwoD3.png}}
 		\hspace{.6in}
	\subfigure[The Object Restores Its Shape With Internal Air Pressure Force]
	{\label{fig:TwoD2}
 		\includegraphics[width=2in]{images/TwoD2.png}}
\caption{Double-layered Two-dimensional Elastic Object filled With Air}
\end{center}
\end{figure*}

In the figure a, the object is deformed from bottom because of the gravity force. If there is no internal air pressure, the object will collapse unless the springs are hard enough to avoid the failure. With the very hard springs, it is difficult to simulate the reality of the elasticity. The real elastic object will squish outwards to restore its shape as described in figure b.  
 
The simplified version of the Ideal Gas Law\cite{mm04}, also known as Clausius Clapeyron Equation, is used to describe such effect:
 
\begin{equation}
\vec{P}V = P\cdot\vec{n}RT \iff \vec{P} = \frac{P\cdot\vec{n}RT}{V}
\end{equation}
where

$\vec{P}$ is the pressure force vector,

$P$ is the pressure value, 

$V$ is the volume of the object, 

$\vec{n}$ is the normal vector to the edges on the object, 

$R$ is the gas constant, 

$T$ is the gas temperature. 

In order to find an estimate pressure inside of the object which will be applied to particles later, we need to calculate the volume of the object. The approximation of the volume calculation is considered to be enough because we only care about the volume in general change. 

To calculate the object volume, we use Gauss Theorem for closed shape object. It replaces the integration over the volume by integration of the surface. The simplified integration of body volume is introduced by Maciej Matyka \cite{mm04}:

\begin{equation}
V = \displaystyle\sum_{i=0}^{i=NUMS-1}\frac{1}{2}|x_{1}-x_{2}|\cdot \vec{n}\cdot length
\end{equation}

where

$V$ is the volume of the object, 

$|x_{1}-x_{2}|$ is the absolute difference of the spring of the start and end particles at axis x,

$\vec{n}$ is the normal vector to this spring at axis x,

$length$ is the spring's length.

The internal air pressure force prevents the object from collapsing when it is compressed by external forces. Moreover, it simulates the object in reality by demonstrating the derivate calculation of the force and volume.  

\paragraph *{Collision Force} is the same method as we inherited from one-dimensional object model, which is to check every particle on the object in each update and to see if it is outside of the pre-defined boundary, such as the walls and floors. In this two-dimensional method, the particles on the outer layer still follow the same method and same pre-defined boundary. However, for the particles on the inner layer, the boundary is constrained to the outer layer instead of the wall and floor. 

\subsection{Result and Summary}
I have modeled a two-dimensional double layered elastic object based on the knowledge from one-dimensional object. The modeling of different springs has been introduced. Moreover, the new force, air pressure force and approximated calculation of the object volume have been discussed also. 
\section{3D}
In this section, a more complicated three-dimensional elastic object is extended from the two-dimensional object. In two-dimensional model, the springs, especial the structural springs' index is the most important key data structure to link up all the particles and reference about the index of the particles. This spring linkage method will still work for the model based on the non-unit sphere geometric modeling method. However, in the other geometric modeling method, the unit sphere modeling, the facets are the key data structure of the linkage to other data structure, such as particles and springs. The reason is because in the later geometric modeling method, each facet on the object is used for subdivision of other facets in each iteration. I will explain in details after the two geometric modeling methods are discussed.

\subsection{Geometric Modeling}
Compared with a two-dimensional object, the three-dimensional object consists the same types of primitives, such as particles, springs, and faces, but extended to z axis. For any particle $i$, the mass, position, velocity, the derivative new position, the derivative new velocity, and the the forces act on it will represented as the following:

$mass_{i} = \left(m_x, m_y, m_z\right)$

$position_{i} = \left(r_x, r_y, r_z\right)$

$velocity_{i} = \left(v_x, v_y, v_z\right)$

$dposition_{i} = \left(dr_x, dr_y, dr_z\right)$

$dvelocity_{i} = \left(dv_x, dv_y, dv_z\right)$

$force_{i} = \left(f_x, f_y, f_z\right)$

\subsubsection{non-uniform ball}

One of the simple non-uniform modeling method to generate a approximate facet sphere uses Polar to cartesian coordinates method. 

\begin{figure*}[h]
\begin{center}
	{\label{fig:ThreeD} \includegraphics[width=2in]{images/ThreeD1.png}}
\caption{Polar Cartesian Coordinates Non-unit Sphere}
\end{center}
\end{figure*}

Consider angle $\theta$ is the angle on $xy-plane$ (around $z-axis$), known as the azimuthal coordinate. The angle $\phi$ is from $z-axis$, known as the polar coordinate. 

Therefore, 

the north pole is $(0, 0, radius)$; 

the south pole is $(0, 0, -radius)$; 

$\theta$ is longitude (eastward positive, westward negative);

$\phi$ is latitude (northward positive, southward negative).

By stepping $\theta$ and $\phi$ in small angles $\Delta\theta$ and $\Delta\phi$ between their bounds as the number of slices and stacks, the spherical coordinates for a particle i can be defined as

$x = \cos\theta \cos\phi$

$y = cos\theta sin\phi$

$z = sin\theta$

where 

$-90 <= \theta <= 90$

$0 <= \phi <= 360$

Any polygonal-facet on the sphere can be represented by four vertices:

$(\theta , \phi, \theta)$

$(\theta+\Delta\theta , \phi, \theta+\Delta\theta)$

$(\theta+\Delta\theta , \phi+\Delta\phi, \theta+\Delta\theta)$

$(\theta , \phi+\Delta\phi, \theta)$

The disadvantage of this non uniform sphere modeling method is that the facets of the sphere do not have approximate 
equal size. The facets become smaller at the poles and bigger in the middle.

 
\subsubsection{uniform ball}
Surface refinement is a simple way for uniform modeling. It is started with a kernel polyhedron, which is a regular polyhedron with faces that are equilateral triangles. I have used an octahedron with bisecting each face at the same time, then finally approach to a sphere according to the desired resolution. 

\begin{figure*}[h]
\begin{center}
	\subfigure[The Initial Octahedron Shape]
	{\label{fig:iteration0} \includegraphics[width=1.5in]{images/iteration0.png}}
	 \hspace{.2in}
	\subfigure[The Unit Facet Sphere Object Iterated Once]
  {\label{fig:iteration1} \includegraphics[width=1.5in]{images/iteration1.png}}
	 \hspace{.2in}
	\subfigure[The Unit Facet Sphere Object Iterated Twice]
  {\label{fig:iteration2} \includegraphics[width=1.5in]{images/iteration2.png}}
\caption{Unit Facet Sphere Generation}
\end{center}
\end{figure*}

In the graphs, the algorithm starts with a regular octahedron. The vertices of the kernel polyhedron are known to lie on the surface of a sphere of radius $r$. Each triangular face of the kernel polyhedron is subdivided by projecting the midpoints of its three edges onto the surface of the sphere. By iterate the first time, each face is split into four faces by bisecting each edge. The number of facets increase by a factor of 4 on each iteration. Four new triangles are defined using the three original points and the three projected points. After the randomly particle and face generated, each particle will be normalized as the distance to the radius so that it will reside on the sphere.

The disadvantages of the unit facet sphere generation algorithm is that it can not generate surfaces of arbitrary resolution. It can be shown that at all levels of recursion particles at the kernel points of the octahedron are connected to four springs. All particles at recursive generated points are connected to six springs. This will result the irregular surface stiffness and might cause the non-spherical shape because the same pressure will displace the regions of surface about the kernel points further than the rest of the surface. 

To solve this problem, either by playing the trick with the air pressure and spring stiffness parameters, so the difference of the force for every particle either connected with four springs, or six springs will be omit. Or, scale the force on the particle connected with six springs.

\subsubsection{Normals} are as important as the role in two-dimensional object simulation. The calculation is important because it will define the direction of the internal air pressure force, either compress the elastic object or expand its volume. In three-dimensional simulation, the normal of a spring in the space position can be represent as
 
\[\left[\begin{array}{c}
{x'} \\
{y'} \\
{z'} \end{array}\right]= 
\left[\begin{array}{cccc} 
cos{90} & -sin{90} & 0 & 0 \\
sin{90} & cos{90} & 0 & 0\\
0 & 0 & 1 & 0 \\
0 & 0 & 0 & 1 \end{array} \right]
\left[\begin{array}{cccc} 
1 & 0 & 0 & 0 \\
0 & cos{90} & sin{90} & 0 \\
0 & -sin{90} & cos{90} & 0 \\
0 & 0 & 0 & 1 \end{array} \right]\]
\[\left[\begin{array}{cccc} 
cos{90} & 0 & -sin{90} & 0 \\
0 & 1 & 0 & 0 \\
sin{90} & 0 & cos{90} & 0\\
0 & 0 & 0 & 1 \end{array} \right]
\left[\begin{array}{c} 
{x_2-x_1} \\
{y_2-y_1} \\
{z_2-z_1} \end{array} \right]\]

Therefore,

\[\left[\begin{array}{c}
{x'} \\
{y'} \\
{z'} \end{array}\right]= \left[\begin{array}{c}
-\left({x_2-x_1}\right)\\
{z_2-z_1} \\
{y_2-y_1} \end{array} \right]\]


\subsection{Algorithm}
\begin {itemize}
\item Step 1: Define a collection of particles to create a closed equilateral triangles shape of the elastic object. We define an octahedron object as the initial object. Six particles with mass value $m_{\left( x, y, z \right)}$, velocity $\vec{v}_{\left(x, y, z\right)}$, derivative velocity $\vec{dv}_{\left(x, y, z\right)}$, the position $\vec{r}_{\left(x, y, z\right)}$, the derivative position $\vec{dr}_{\left(x, y, z\right)}$.
\item Step 2: All the particles have the default gravity force $\vec{F}^{g}$ points down to the opposite of y axis.
\item Step 3: Connect the particles with the structural springs according to the edge order of the octahedron to make an inner layer of the three-dimensional object. Each particle is separated equidistantly from its neighbors.
\item Step 4: Check if there is need of subdivision to approach a more spherical object.
\item Step 5: Each iteration, more particles are generated, more structural springs are added, and more faces are approaching the object to a unit facet sphere.
\item Step 6: Repeat Step 1 to 5 to create an outer layer two times bigger than the inner layers.
\item Step 7: Loop through the number of structural springs to add the same number of radium springs according to the linkage of the inner and outer particles.
\item Step 8: Loop through the number of structural springs to add the same number of shear left springs and shear right springs according to the linkage of the inner and outer particles. 
\item Step 9: Split object into regions, integrate density and weight in each region to modify mass. The current system considers the particle weights are all same. In the future model, the density and weight of the particles can be vary in order to get the non-unit motion.
\item Step 10: Changing the spring constants for the different types of springs of the system. Also, different density effects can be realized. The consequence is that the force of each particle varies from the different compression of springs.
\item Step 11: Initialize density as gas, liquid, or rubber inside of the body and introduce some simple physics to describe it. In the current system, only air pressure material is considered and only pressure equation will be used for this extra force computation.
\item Step 12: Calculate all forces accumulated on the each inner and outer layer particle except air pressure force. 
\item Step 13: Calculate volume of the inner layer of the elastic object. 
\item Step 14: Calculate volume of the outer layer of the elastic object. 
\item Step 15: Calculate the normal of springs on each triangular face to define the pressure force direction.
\item Step 16: Calculate the force from the internal air pressure by multiplying the result by field of the face.
\item Step 17: Accumulate finally pressure force to each particle.
\item Step 18: Integration the object's momentum motion by calculating the derivative velocity and its new position for each particle.
\item Step 19: Resolve collision detection and response and define the updated position.
\item Step 20: Loop through Step 12.  
\end{itemize}

\subsection{Forces} 

Accumulation of forces on a three-dimensional object particle are similar to forces applied on the two-dimensional one, such as the gravity, the mouse dragging force, the collision force as the external forces and the spring hook and damping forces, the air pressure force as internal forces. The only difference from the forces on two-dimensional object is that he forces on three-dimensional object are extended to axis z.

\subsection{Result and Summary}
In this section, I not only introduce the two geometric modeling methods to make a sphere, but also explain how the calculation of the spring normal in three-dimension differs from two-dimension. Moreover, I list the algorithm in more detailed steps to explain how the system works.
 


==> otherfeatures.tex <==
\chapter{Other Features}
\parskip        1.5ex plus 1ex minus 0.5ex
\parindent      0em
\label{chapt:other features}
\index{Other features}

\section{Other related aspects}
\section{Collision Detection}
Track the movements of the soft body objects and detect when they collide. The calculation is expensive if test all object for collisions with all other objects. sqr(n(n-1)/2 tests) with n objects. However, efficient algorithm will sort roughly first to determine the objects that definitely does not collide in order to reduce the calculation. 

\subsection{Collision objects}

-	Closed convex: line between two points inside the object never crosses the surface of the object, fast to check collision

-	Closed concave: split it up to convex objects

-	Arbitrary meshes: non-closed mesh placed in 3D

\subsection{Collision Methods}
\begin{diamonds}
\item Penalty force methods: easy to implement, hard to get robust result.\cite{MW88}\cite{PB88}
\item Analytical methods: by solving equations globally, stiffness problems are eliminated.
\item Micro collision methods
\item When interact with a sphere, check each point on the object to see if it is inside of the sphere, if it is, move it to the nearest point of the sphere.
\item interact with a floor, check each point on the object to see if it is below the floor, if it is below the floor, then move it back to the surface.
\end {diamonds}

This elastic object simulation system is using the last method, check the floor, or can be said as BEM (Boundary Element Method). It is the most efficient computation method and can achieve desired deformation result.

$${P}_{osition\_point} = {P}_{osition\_center\_sphere} + ForceVector$$

where

$$ForceVector = \frac{{P}_{osition\_point}-{P}_{osition\_center\_sphere}}{{D}_{istance\_point\_to\_center\_of\_sphere}}\cdot radius$$

\subsection{Detection Methods}
Broad phase, pairs of objects are excluded if they are far away to each other so that it is impossible for them to interact with each other...

-	AABB-adjacent bounding boxes, adjacent to x, y, z axis

-	OBB-Object bounding boxes

-	Group objects-different types of objects only need to interact with certain other type

Narrow phase, all surface are tested for collision and a detailed collision list is created.

-	Impulse-momentum

-	Impact

-	Linear and angular impulse

-	Friction

bounding objects method: bounding box, bounding ball, and bounding ellipsoid

For the volume of ellipsoid with ${r}_{x}$, ${r}_{y}$, and ${r}_{z}$ radiuses 

$$V_{el}=\left(\frac{4}{3}\right)\cdot \pi \cdot {r}_{x}{r}_{y}{r}_{z}$$

\subsection{Hardware related}

Faster processor allows heavy and complicated animation. Physical simulation runs on computer's motherboard processors; visualization of obejcts animation is done by 3D graphics cards.

Current 3d graphics cards limit both in
- number of polygon triangles displayed simultaneously
- bandwidth between motherboard and the graphics card
Modern graphics cards can display a significantly larger amount of triangles per frame than it is possible to feed the card, maintaining a decent frame rate [M 02]. This results in that it is more efficient to upload the total geometry of a huge landscape grid on the graphics card in the initial simulation setup phase, instead of creating a software level of detail algorithm within your application that minimizes the number of polygons. This may change as hardware continues to develop.

These restrictions affect the possibilities of simulating deformable object physics. Examples include deformable landscapes and cloth techniques, which may involve sending thousands of updated polygon coordinates to the graphics card each new time frame.

More and more algorithms are integrated on the graphics cards used by professional 3D modelers and gamers. The new generations of graphics cards support writing your own small programs, upload them to, and let them be run by the graphics card instead of the processor(s) on the motherboard.
Performance exemplified
Roughly, a modern 2 GHz Pentium 4 can manage about 60-70 rigid bodies with 10-20 fps. For most VR applications, a maximum of only 20 of the total CPU-time can be used for physics. The complexity of the problem generally increases execution time quadratic in relation to the number of bodies and attached rules. There are implementation methods like Featherstone's algorithm [F 83][F 87], which can reduce the time/complexity factor from N2 to N*log (N), and for some cases even N.

Software or hardware
According to Kenneth Holmlund at VR-Lab, most physical simulation problems are solved by software and it will remain that way for quite some time since it is hard to standardize physic simulation methods. Today's processors are quite specialized on technical calculations, which is what physics demand. MMX, SIMD, 3DNOW and similar processor architectures are important for optimization, but are very rough and tedious tools. Even new advanced C++ tools, which optimize matrix calculations, are too complicated for practical use.

Parts of polygon handling could be done on the graphics cards eventually, mixing OpenGL functions with physics. Collision detection culling could theoretically be done by hardware, but the more complex integrations will take time to standardize enough. Constructing a "physics processor" at this point would be pointless, says Holmlund. There have been discussions about it but CPU manufacturer Intel concluded that their ordinary CPUs are still cheaper thanks to the enormous volume.
 



\subsection{Lighting}

Calculate vertex normals as the average of the face normals, and use them to add lighting effects.


Collision and Detection:

Collision detection\index{collision detection} and their response for soft bodies are extremely complex.
When an object hit on a plane, all the vertex of the object will be tested. There will be world boundaries. There is a initial velocity and the object can bounce off of the boundaries. Need to apply forces and acceleration to particles dynamically.
When two objects collide together...

The simplest form of collision detection is point-to-plane collision. Use dot product to determine whether a point has collided with a plane.

Diagram:

Particle x with a velocity vector V is moving towards plane P with a normal N.
If (X-P). N <e, where e is some small threshold near zero; then collision occurred.
If <-e; then the particle has passed through the wall, wrong result.

Also, when the object bounces around, it is going to collide on the boundary walls.



\section{Testing Cases}
There are many physical parameters Sometimes need to play with the coefficients. to get the best testing results, or reduce the integrator time steps to avoid devergence if less heavy calculation can already achieve a decent result.

Further to the 2D soft body I have achieved, now I have built a few of different kind of 3D soft balls using spring mass and pressure model.  I have used 2 different sets of parameters P, V, F, M, K, D... to try to investigate the non-uniform physical properties of a soft ball.
Problem encountered:

For the 2 separate soft balls with 2 sets of different physical parameters, they run well as expected. Yet, when being connected by springs between their corresponding points from inner ball to outer ball, the deformation of the combined body, a concentric ball become uncontrolled and non-expected.  The reason, at the first place, is because the  3D asymmetry when building the ball from their primary points.

\begin{itemize}
\item Moving the position
\item Adding force or pressure of the object, if the inside pressure is too high with small volume object, the deformation becomes unrealistic. The only solution to decrease this deformation is to increase the stiffness of the deformed springs.
\item Damping and elasticity factors value should be carefully selected.
when constant value of elasticity or damping are set too high, the simulation might "blow up", means the mass points on object will toward infinity. To constrian and terminate the simulation when it detects the point coordinates have become extremely large. Tips to avoid: decrease the value of the leasticity/damping parameter, or decrease the value of timestep.
\item the higher the stiffness, the higher the cost of the algorithm 
\item the number of particles and springs increase, the cost of computation increases
\item Collision detection
\end{itemize}

\subsection{ODE Integrators}

\begin{itemize}
\item The error varies with the time step. With smaller time step, all the three solvers give the approximately results. However, with larger step, Euler Integrator and Midpoint Integrator start to diverge; RK4 Integrator does not. If the step is extremely large, all the integrators will diverge, the RK4 will be the last one to be diverged.
\item test efficiency
\item test stability, the system is instability when the drag constant is very high and time step is too high. If the time step is small, the mass is almost resting.
\item set spring constant is very high = 1000kg/s or .1kg/s with mass 5kg. 
\item time step = .01, .1, 1. m = 5kg, ks = 15kg/s, kd = 1 kg/s. rest length = 5 m.
\end{itemize} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> others.tex <==
\chapter{Others}
\parskip        1.5ex plus 1ex minus 0.5ex
\parindent      0em
\label{chapt:others}
\index{Others}

\section{Testing Cases}
\section{Related Features}
Hardware related. Faster processor
\section{future work}

==> summary.tex <==
\clearpage
\section{Summary}
\thispagestyle{plain}

Conclusion:
- Pressure model of soft body behavior is fast (a couple of ms for thousands of vertices)
- gives good soft behavior in real time
- It is easy for implementation

Future work:
-	implicit integration (not for real time)
-	Monte Carlo volume calculation
-	self collision detection  and response (bounding box)
